StepFun-Formalizer: Unlocking the Autoformalization Potential of LLMs through Knowledge-Reasoning Fusion

Autoformalization aims to translate natural-language mathematical statements into a formal language. While LLMs have accelerated progress in this area, existing methods still suffer from low accuracy. We identify two key abilities for effective autoformalization: comprehensive mastery of formal-language domain knowledge, and reasoning capability of natural language problem understanding and informal-formal alignment. Without the former, a model cannot identify the correct formal objects; without the latter, it struggles to interpret real-world contexts and map them precisely into formal expressions. To address these gaps, we introduce ThinkingF, a data synthesis and training pipeline that improves both abilities. First, we construct two datasets: one by distilling and selecting large-scale examples rich in formal knowledge, and another by generating informal-to-formal reasoning trajectories guided by expert-designed templates. We then apply SFT and RLVR with these datasets to further fuse and refine the two abilities. The resulting 7B and 32B models exhibit both comprehensive formal knowledge and strong informal-to-formal reasoning. Notably, StepFun-Formalizer-32B achieves SOTA BEq@1 scores of 40.5% on FormalMATH-Lite and 26.7% on ProverBench, surpassing all prior general-purpose and specialized models.

==> figures/1_introduction/previous_formalizer_bad_case_2.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tcolorbox}[
        colback=white,      % 背景色
        colframe=black,     % 边框色
        arc=0pt,            % 边框直角
        boxrule=1pt,        % 边框粗细
        width=0.9\linewidth,% 宽度
        center,             % 居中
        left=5mm,           % 左边距
        right=10mm,          % 右边距
        top=3mm,            % 上边距
        bottom=3mm,         % 下边距
        breakable           % 允许跨页
    ]
    \textbf{Informal Problem}: The real numbers $x, y, z$ satisfy $0 \leq x \leq y \leq z \leq 4$. If their squares form an arithmetic progression with common difference $2$, determine the minimum possible value of $|x-y|+|y-z|$.
    
    Prove that the answer is: $4-2\sqrt{3}$.

    \medskip

\textbf{Formal Statement (Human)}:    
\begin{lstlisting}[language=lean,basicstyle=\ttfamily,frame=none,escapechar=!]
open Real
theorem omni_theorem_637 : IsLeast {n : ℝ | ∃ x y z, 0 ≤ x ∧ x ≤ y ∧ y ≤ z ∧ z ≤ 4 ∧ n = abs (x - y) + abs (y - z) ∧ y^2 - x^2 = !\colorbox{shallowBlue}{2}! ∧ z^2 - y^2 = !\colorbox{shallowBlue}{2}!} (4 - 2 * sqrt 3) := by sorry
\end{lstlisting}

    \medskip

\textbf{Formal Statement (\KMAuto)}:    
\begin{lstlisting}[language=lean,basicstyle=\ttfamily,frame=none,escapechar=!]
theorem my_favorite_theorem : IsLeast { |x - y| + |y - z| | (x : ℝ) (y : ℝ) (z : ℝ) (h₀ : 0 ≤ x) (h₁ : x ≤ y) (h₂ : y ≤ z) (h₃ : z ≤ 4) (h₄ : ∃ d, x^2 = y^2 - !\colorbox{shallowBlue}{2 * d}! ∧ y^2 = z^2 !\colorbox{shallowRed}{+}! !\colorbox{shallowBlue}{2 * d}!) } (4 - 2 * √3):= by sorry
\end{lstlisting}

    \end{tcolorbox}

% \caption{TODO \textbf{A case study to demonstrate the lack of domain knowledge and informal-formal misalignment.} \KMAuto makes the following mistakes: (1) It misinterpreted the price of twelve donuts as the price of a single donut (\colorbox{shallowRed}{red}). (2) it omits to declare the type of total payment ($\mathtt{x}$) as a real number, which will cause an type coercion error for 7.49 in Lean 4 (\colorbox{shallowBlue}{blue}). The reasoning process shows that \modelname can avoid these mistakes.} 
% 1. 错误地翻译了公差为2
% 2. 公差符号不正确
% 3. 没有必要的条件命名
\label{fig:bad_case_2}

\end{figure*}



==> figures/1_introduction/previous_formalizer_bad_case_3.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tcolorbox}[
        colback=white,      % 背景色
        colframe=black,     % 边框色
        arc=0pt,            % 边框直角
        boxrule=1pt,        % 边框粗细
        width=0.9\linewidth,% 宽度
        center,             % 居中
        left=5mm,           % 左边距
        right=10mm,          % 右边距
        top=3mm,            % 上边距
        bottom=3mm,         % 下边距
        breakable           % 允许跨页
    ]
    \textbf{Informal Problem}: Find all values of $x$ that satisfy the following equation:
    $\left|\left(x^2+4 \cdot x+9\right)+(2 \cdot x-3)\right|=\left|x^2+4 \cdot x+9\right|+|2 \cdot x-3|$. 
    Prove that the answer is: The final answer: $x\ge\frac{3}{2}$.

    \medskip

\textbf{Formal Statement (\modelname)}:    
\begin{lstlisting}[language=lean,basicstyle=\ttfamily,frame=none,escapechar=!]
theorem my_favorite_theorem (x : ℝ) : |x^2 + 4 * x + 9 + 2 * x - 3| = |x^2 + 4 * x + 9| + |2 * x - 3| ↔ x ≥ 3 / 2 := by   sorry
\end{lstlisting}

    \medskip

\textbf{Formal Statement (\KMAuto)}:    
\begin{lstlisting}[language=lean,basicstyle=\ttfamily,frame=none,escapechar=!]
theorem my_favorite_theorem (x : ℝ) : abs (!\colorbox{shallowRed}{abs}! (x^2 + 4 * x + 9) + !\colorbox{shallowRed}{abs}! (2 * x - 3)) = abs (x^2 + 4 * x + 9) + abs (2 * x - 3) ↔ x ≥ 3 / 2 := by sorry
\end{lstlisting}

    \end{tcolorbox}

% \caption{TODO \textbf{A case study to demonstrate the lack of domain knowledge and informal-formal misalignment.} \KMAuto makes the following mistakes: (1) It misinterpreted the price of twelve donuts as the price of a single donut (\colorbox{shallowRed}{red}). (2) it omits to declare the type of total payment ($\mathtt{x}$) as a real number, which will cause an type coercion error for 7.49 in Lean 4 (\colorbox{shallowBlue}{blue}). The reasoning process shows that \modelname can avoid these mistakes.} 
% 1. $\left|\left(x^2+4 \cdot x+9\right)+(2 \cdot x-3)\right|$翻译错误
\label{fig:bad_case_2}

\end{figure*}



==> figures/1_introduction/previous_formalizer_bad_case_4.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tcolorbox}[
        colback=white,      % 背景色
        colframe=black,     % 边框色
        arc=0pt,            % 边框直角
        boxrule=1pt,        % 边框粗细
        width=0.9\linewidth,% 宽度
        center,             % 居中
        left=5mm,           % 左边距
        right=10mm,          % 右边距
        top=3mm,            % 上边距
        bottom=3mm,         % 下边距
        breakable           % 允许跨页
    ]
    \textbf{Informal Problem}: Two thousand points are given on a circle. Label one of the points 1. From this point, count 2 points in the clockwise direction and label this point 2. From the point labeled 2, count 3 points in the clockwise direction and label this point 3. (See figure.) Continue this process until the labels $1,2,3\dots,1993\,$ are all used. Some of the points on the circle will have more than one label and some points will not have a label. What is the smallest integer that labels the same point as 1993? Prove that the answer is: 118

    \medskip

\textbf{Formal Statement (Human)}:    
\begin{lstlisting}[language=lean,basicstyle=\ttfamily,frame=none,escapechar=!]
theorem my_favorite_theorem : IsLeast {n | 0 < n ∧ (n * (n + 1)) / 2 ≡ 1993 * 1994 / 2 [MOD 2000]} 118 := by sorry
\end{lstlisting}

    \medskip

\textbf{Formal Statement (\KMAuto)}:    
\begin{lstlisting}[language=lean,basicstyle=\ttfamily,frame=none,escapechar=!]
theorem my_favorite_theorem (a : ℕ → ℕ) (ha0 : a 0 = !\colorbox{shallowBlue}{1993}!) (han : ∀ n, a (n + 1) = (a n + (n + 1)) % 2000) : IsLeast {n | a n = a !\colorbox{shallowRed}{0}!} 118 := by sorry
\end{lstlisting}

    \end{tcolorbox}

% \caption{TODO \textbf{A case study to demonstrate the lack of domain knowledge and informal-formal misalignment.} \KMAuto makes the following mistakes: (1) It misinterpreted the price of twelve donuts as the price of a single donut (\colorbox{shallowRed}{red}). (2) it omits to declare the type of total payment ($\mathtt{x}$) as a real number, which will cause an type coercion error for 7.49 in Lean 4 (\colorbox{shallowBlue}{blue}). The reasoning process shows that \modelname can avoid these mistakes.} 
% 1. 数列起始位置不正确
% 2. 集合条件不正确
\label{fig:bad_case_2}

\end{figure*}



==> sections/5_implementation_details.tex <==
\section{Implementation Details}
\label{sec:implementation_details}


==> tables/1_introduction/error_type_gpt4o_vs_human.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{1mm}
    %\fontsize{9}{11}\selectfont
    \begin{tabular}{cc|cccc}
    \toprule
    \multicolumn{1}{c}{Model} & Evaluation & Correct & NLU & IFM & Other \\
    \midrule
    Kimina     & GPT-4o             & 28.77      & 36.99  & 28.77  & 5.47    \\
    Kimina     & Human              & 35.71      & 35.71  & 24.29  & 4.29    \\
    \modelname   & GPT-4o           & 45.76      & 20.34  & 20.34  & 13.56   \\
    \modelname   & Human            & 50.00      & 26.79  & 16.07  & 7.14    \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Effectiveness validation of GPT-4o in autoformalization type error analysis.} We randomly select the generations of each LLM for 50 problems and compare the errors (\%) between GPT-4o and humans, where NLU refers to the error caused by Natural Language Understanding and IFM refers to the error caused by Informal-formal Misalignment.}
    %It indicates that the proportion of the two error types assessed by GPT-4o is similar to that of human evaluation.}
    \label{tab:error_type_gpt4o_vs_human}
\end{table}


==> tables/1_introduction/syntax_error_in_general_llms.tex <==
\begin{table}
    \centering
    %\setlength{\tabcolsep}{1mm}
    %\fontsize{9}{11}\selectfont
    \begin{tabular}{lc}
    \toprule
    \multicolumn{1}{c}{Model}                 & Syntactic Accuracy \\
    \midrule
    \multicolumn{2}{l}{\it (General-purpose Models)}                 \\
    Gemini-2.5-thinking          & 61.33              \\
    DeepSeek-R1                  & 77.78              \\
    OpenAI o3-pro                & 82.65              \\
    Claude4-thinking             & 84.25              \\
    \RRD-7B                      & 37.06              \\
    QwQ-32B                      & 49.99              \\
    \midrule
    \multicolumn{2}{l}{\it (Models specialized for Autoformalization)}                 \\
    \KMAuto-7B                                & 85.19              \\
    \modelname-7B (ours)                      & \underline{85.32} \\
    \modelname-32B (ours)                     & \textbf{88.51}              \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Syntactic accuracy (\%) of general-purpose vs. specialized LLMs in autoformalization.} We evaluate the syntax accuracy of the generation results from mainstream general-purpose models \cite{gemini, deepseekr1, o3-pro, claude4-thinking, qwq32b} and autoformalization specialized models \cite{Prover-Kimina} on three benchmarks using the Lean 4 REPL \cite{repl}.}
    \label{tab:syntax_error_in_general_llms}
\end{table}


==> tables/6_experiments/main_results_bk.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{0.8mm}
\fontsize{9}{11}\selectfont

\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{FormalMATH-Lite} & \multicolumn{2}{c}{ProverBench} \\
&  BEq@1 & BEq@16 & BEq@1 & BEq@16 \\
\midrule
\multicolumn{5}{l}{(\textit{General-purpose Models})} \\
OpenAI o3-pro        & 22.6 & 35.5 & 24.7 & \underline{36.2} \\
% OpenAI o4-mini       & 19.2 & 31.3 & 23.9 & \textbf{38.5}  \\
Claude4-thinking     & 20.8 & 32.2 & 24.4 & 35.6 \\
Gemini-2.5-thinking  & 17.8 & 31.3 & 20.1 & \textbf{36.8} \\
\RR-671B             & 18.4 & 31.3 & 23.5 & 34.5 \\
QwQ-32B              & 14.0 & 25.4 & 15.1 & 27.6  \\
DeepSeek-R1-Distill-7B              & 5.2  & 14.6 & 5.4  & 18.4  \\
\midrule
\multicolumn{5}{l}{(\textit{Specialized Models})} \\
LeanFormalizer-PPO-7B           & 18.7 & 24.0 & 12.4 & 18.4 \\
LeanFormalizer-SFT-7B           & 18.9 & 23.3 & 18.4 & 26.4  \\
LeanFormalizer-CoT-7B           & 13.5 & 29.9 & 8.5 & 28.2  \\
Herald-Translator-7B             & 13.6 & 24.7 & 8.2 & 27.0  \\
Goedel-Sonnet-32B  & 18.7 & 29.2 & 13.6 & 27.6  \\
Goedel-LW-32B      & 15.1 & 26.4 & 5.0 & 12.1  \\
Kimina-Auto-7B                    & 35.1 & \textbf{60.2} & 13.3 & 25.3  \\%
\midrule
\rowcolor[rgb]{0.925,0.925,0.925} \multicolumn{5}{l}{(\textit{Ours})} \\
\rowcolor[rgb]{0.925,0.925,0.925} \modelname-7B & \underline{42.3} & \textbf{60.2} & \underline{24.9} & 31.6 \\%
\rowcolor[rgb]{0.925,0.925,0.925} \modelname-32B & \textbf{43.3} & \underline{59.5} & \textbf{26.0} & 35.6 \\
\bottomrule
\end{tabular}%
\caption{\textbf{BEq@1 (\%) results of \modelname and baselines on FormalMATH-Lite and ProverBench.} ``Goedel-Sonnet/LW-32B'' refers to Goedel-Formalizer-32B-SonnetAnnotated/LeanWorkbookAnnotated.
``Kimina-Auto-7B'' refers to \KMAuto-7B.}
\label{tab:main_results}
\end{table}


==> tables/6_experiments/main_results_complete.tex <==
\begin{table*}[h]
%\setlength{\tabcolsep}{0.8mm}
\fontsize{9}{11}\selectfont
\centering

\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{FormalMATH-Lite} & \multicolumn{2}{c}{ProverBench} & \multicolumn{2}{c}{CombiBench} \\
&  BEq@1 & BEq@16 & BEq@1 & BEq@16 & BEq@1 & BEq@16 \\
\midrule
\multicolumn{7}{l}{(\textit{General-purpose Models})} \\
OpenAI o3-pro        & 22.6 & 35.5 & 24.7 & 36.2 & \underline{9.0} & 16.0 \\
%OpenAI o4-mini       & 19.2 & 31.3 & 23.9 & \textbf{38.5}  \\
Claude4-thinking     & 20.8 & 32.2 & 24.4 & 35.6 & \textbf{9.7} & \underline{18.0} \\
Gemini-2.5-thinking  & 17.8 & 31.3 & 20.1 & 36.8 & 8.9 & \underline{18.0} \\
\RR-671B             & 18.4 & 31.3 & 23.5 & 34.5 & 8.1 & \textbf{20.0} \\
% QwQ-32B              & 14.0 & 25.4 & 15.1 & 27.6  \\
DeepSeek-R1-Distill-7B              & 5.2  & 14.6 & 5.4  & 18.4 & 0.4 & 2.0  \\
\midrule
\multicolumn{7}{l}{(\textit{Specialized Models})} \\
LeanFormalizer-PPO-7B           & 18.7 & 24.0 & 12.4 & 18.4 & 0.1 & 1.0 \\
LeanFormalizer-SFT-7B           & 18.9 & 23.3 & 18.4 & 26.4 & 4.8 & 8.0 \\
LeanFormalizer-CoT-7B           & 13.5 & 29.9 & 8.5  & 28.2 & 2.1 & 9.0 \\
Herald-Translator-7B            & 13.6 & 24.7 & 8.2  & 27.0 & 1.3 & 5.0 \\
Goedel-Formalizer-SonnetAnnotated-32B               & 18.7 & 29.2 & 13.6 & 27.6 & 3.4 & 10.0 \\
Goedel-Formalizer-LeanWorkbookAnnotated-32B                   & 15.1 & 26.4 & 5.0  & 12.1 & 0.3 & 2.0 \\
\KMAuto-7B                  & 35.1 & \underline{60.2} & 13.3 & 25.3 & 2.6 & 6.0 \\%
\midrule
\rowcolor[rgb]{0.925,0.925,0.925} \multicolumn{7}{l}{(\textit{Ours})} \\
\rowcolor[rgb]{0.925,0.925,0.925} \modelname-7B  & \underline{38.3} & \textbf{61.2} & \underline{25.1} & \underline{37.9} & 5.2 & 11.0 \\
\rowcolor[rgb]{0.925,0.925,0.925} \modelname-32B & \textbf{40.5} & 59.3 & \textbf{26.7}    & \textbf{38.5} & 6.9 & 14.0 \\
\bottomrule
\end{tabular}%
\caption{\textbf{BEq@1 and BEq@16 (\%) results of \modelname and baselines on three benchmarks.}}
\label{tab:main_results}
\end{table*}


==> utils/lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% Anything between $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, constant, constants,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class,
raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const,
partial, mut, where, macro, syntax, deriving,
return, try, catch, for, macro_rules, declare_syntax_cat, abbrev},

% Sorts
morekeywords=[2]{Sort, Type, Prop},

% tactics, list taken from lean-syntax.el
morekeywords=[3]{
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction,
constructor, injection,
induction,
},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{∣}{{\ensuremath{\mathrm{\mid}}}}1
{⧸}{{\ensuremath{\mathrm{/}}}}1
{⋂}{{\ensuremath{\mathrm{\bigcap}}}}1
{__N}{{\ensuremath{\mathcal{N}}}}1

{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt{}}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{ₚ}{{\ensuremath{_p}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\color{symbolcolor}\$}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{<|>}{{\color{symbolcolor}<|>}}1
{<\$>}{{\color{symbolcolor}<\$>}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=false,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the beginning of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize },

}

